Free Hunch: Denoiser Covariance Estimation for Diffusion Models Without Extra Costs

The covariance for clean data given a noisy observation is an important quantity in many training-free guided generation methods for diffusion models. Current methods require heavy test-time computation, altering the standard diffusion training process or denoiser architecture, or making heavy approximations. We propose a new framework that sidesteps these issues by using covariance information that is available for free from training data and the curvature of the generative trajectory, which is linked to the covariance through the second-order Tweedie's formula. We integrate these sources of information using (i) a novel method to transfer covariance estimates across noise levels and (ii) low-rank updates in a given noise level. We validate the method on linear inverse problems, where it outperforms recent baselines, especially with fewer diffusion steps.

==> fig/covariance_approximation/posterior_prior.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={Prior p(x₀) with Likelihood p(y|x₀)},
x grid style={darkgray176},
xlabel={X},
xmin=-4, xmax=4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Y},
ymin=-4, ymax=4,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-6.83870967741935, xmax=15.8709677419355, ymin=-5.32450331125828, ymax=5.27152317880795] {posterior_prior-004.png};
\addplot [draw=none, draw=red]
table{%
x  y
-1.74313297684629 -1.09090912342072
-1.76864659217108 -1.01010096073151
-1.78622896242228 -0.929292917251587
-1.79688910027464 -0.848484873771667
-1.80122263633433 -0.767676770687103
-1.79946842127389 -0.686868667602539
-1.79152979003556 -0.60606062412262
-1.7769666999006 -0.525252521038055
-1.75495389696644 -0.444444447755814
-1.73737370967865 -0.396717551877842
-1.72586028958546 -0.363636374473572
-1.68969921271444 -0.282828271389008
-1.65656566619873 -0.224860627033221
-1.64344203352248 -0.202020198106766
-1.58727304803294 -0.121212124824524
-1.57575762271881 -0.106878350112338
-1.51855709738062 -0.0404040440917015
-1.4949494600296 -0.016252018991976
-1.43275760225123 0.0404040440917015
-1.41414141654968 0.0560664358675098
-1.33333337306976 0.114611529885261
-1.32255048368963 0.121212124824524
-1.25252521038055 0.163410793365699
-1.17171716690063 0.200988237295999
-1.16897432344671 0.202020198106766
-1.09090912342072 0.232792340246537
-1.01010096073151 0.255921188749604
-0.929292917251587 0.271599547572197
-0.848484873771667 0.280721690159996
-0.793271674945034 0.282828271389008
-0.767676770687103 0.283955955489235
-0.739654455396937 0.282828271389008
-0.686868667602539 0.280990283592606
-0.60606062412262 0.27215171391775
-0.525252521038055 0.256787918594234
-0.444444447755814 0.234023603745113
-0.363636374473572 0.202516650991956
-0.362587507015271 0.202020198106766
-0.282828271389008 0.165357919653617
-0.20908745297672 0.121212124824524
-0.202020198106766 0.116917979246685
-0.121212124824524 0.0590866061511772
-0.0988960232800097 0.0404040440917015
-0.0404040440917015 -0.0125747013423628
-0.0130823410430516 -0.0404040440917015
0.0404040440917015 -0.102238571452933
0.0557070330171809 -0.121212124824524
0.111633686413478 -0.202020198106766
0.121212124824524 -0.218611436357328
0.158048491538539 -0.282828271389008
0.194010582969693 -0.363636374473572
0.202020198106766 -0.386549508010962
0.223415026723592 -0.444444447755814
0.245281808037281 -0.525252521038055
0.259748206276833 -0.60606062412262
0.267634070156817 -0.686868667602539
0.269376637027683 -0.767676770687103
0.265071870970438 -0.848484873771667
0.254482561370944 -0.929292917251587
0.237016844580782 -1.01010096073151
0.211672570525063 -1.09090912342072
0.202020198106766 -1.11477845575574
0.180072687567912 -1.17171716690063
0.139567960108191 -1.25252521038055
0.121212124824524 -1.28262500509905
0.0898501417140347 -1.33333337306976
0.0404040440917015 -1.39889808913574
0.0282036245937653 -1.41414141654968
-0.0404040440917015 -1.48828086957432
-0.0472714640311111 -1.4949494600296
-0.121212124824524 -1.56020223974384
-0.141838907966625 -1.57575762271881
-0.202020198106766 -1.61898491450888
-0.266662248669916 -1.65656566619873
-0.282828271389008 -1.66592934957474
-0.363636374473572 -1.7049772622133
-0.444444447755814 -1.73413678708921
-0.456211529228565 -1.73737370967865
-0.525252521038055 -1.7578683804505
-0.60606062412262 -1.77421146287987
-0.686868667602539 -1.78361340059821
-0.767676770687103 -1.78659749018417
-0.848484873771667 -1.78332760658411
-0.929292917251587 -1.77362412234265
-1.01010096073151 -1.75694653913752
-1.07521109375078 -1.73737370967865
-1.09090912342072 -1.73299709793132
-1.17171716690063 -1.70343161742527
-1.25252521038055 -1.66387992612027
-1.26507000791467 -1.65656566619873
-1.33333337306976 -1.61658419784147
-1.38985133136304 -1.57575762271881
-1.41414141654968 -1.55732040452272
-1.4844675737904 -1.4949494600296
-1.4949494600296 -1.48471207789134
-1.55996868662366 -1.41414141654968
-1.57575762271881 -1.39431144137558
-1.62156419181469 -1.33333337306976
-1.65656566619873 -1.27647029882181
-1.67111625269845 -1.25252521038055
-1.71184525102584 -1.17171716690063
-1.73737370967865 -1.10519743834624
-1.74313297684629 -1.09090912342072
};
\addplot [draw=none, draw=red]
table{%
x  y
-1.50028899360728 -0.929292917251587
-1.51569265755879 -0.848484873771667
-1.52195455172877 -0.767676770687103
-1.51941961567662 -0.686868667602539
-1.5079485273424 -0.60606062412262
-1.4949494600296 -0.555355273855511
-1.48731622314033 -0.525252521038055
-1.45713379417588 -0.444444447755814
-1.4149698209547 -0.363636374473572
-1.41414141654968 -0.362339250325931
-1.35938299899071 -0.282828271389008
-1.33333337306976 -0.252007665762537
-1.28524173075422 -0.202020198106766
-1.25252521038055 -0.172542906525804
-1.1836632907399 -0.121212124824524
-1.17171716690063 -0.113054738886363
-1.09090912342072 -0.0681036223485098
-1.02280102371973 -0.0404040440917015
-1.01010096073151 -0.0353342192602128
-0.929292917251587 -0.0122514097519137
-0.848484873771667 0.00117896497609538
-0.767676770687103 0.00570458542909158
-0.686868667602539 0.00157449806971211
-0.60606062412262 -0.0114383803976388
-0.525252521038055 -0.0340582535110374
-0.509154695136402 -0.0404040440917015
-0.444444447755814 -0.0663709688018337
-0.363636374473572 -0.110704855770792
-0.348127431179368 -0.121212124824524
-0.282828271389008 -0.16946593127786
-0.246457630613224 -0.202020198106766
-0.202020198106766 -0.247867934255099
-0.172303819521344 -0.282828271389008
-0.121212124824524 -0.356535128139735
-0.116654433470831 -0.363636374473572
-0.0745601435259431 -0.444444447755814
-0.0444274932081906 -0.525252521038055
-0.0404040440917015 -0.541028225590839
-0.0236587189525747 -0.60606062412262
-0.0122224223484855 -0.686868667602539
-0.00969518687742501 -0.767676770687103
-0.015938094242072 -0.848484873771667
-0.0312951109759372 -0.929292917251587
-0.0404040440917015 -0.959274331160936
-0.0558167049615634 -1.01010096073151
-0.0907412951588713 -1.09090912342072
-0.121212124824524 -1.14393442719687
-0.138275098138448 -1.17171716690063
-0.200857651277172 -1.25252521038055
-0.202020198106766 -1.25381170870171
-0.282828271389008 -1.33182439866572
-0.284698341898904 -1.33333337306976
-0.363636374473572 -1.39052838672969
-0.405537557423586 -1.41414141654968
-0.444444447755814 -1.43490542167443
-0.525252521038055 -1.46743152288302
-0.60606062412262 -1.48938364677279
-0.641141721418197 -1.4949494600296
-0.686868667602539 -1.50243538354679
-0.767676770687103 -1.50668341240497
-0.848484873771667 -1.50202841572815
-0.890451650750952 -1.4949494600296
-0.929292917251587 -1.48859472076597
-1.01010096073151 -1.46619318022421
-1.09090912342072 -1.43314611785625
-1.12617558482252 -1.41414141654968
-1.17171716690063 -1.38820518453463
-1.24685539392629 -1.33333337306976
-1.25252521038055 -1.32871842506829
-1.3307868109307 -1.25252521038055
-1.33333337306976 -1.24959481744544
-1.39341558472631 -1.17171716690063
-1.41414141654968 -1.13775069942149
-1.44092582903761 -1.09090912342072
-1.47590830911368 -1.01010096073151
-1.4949494600296 -0.946944936886047
-1.50028899360728 -0.929292917251587
};
\addplot [draw=none, draw=red]
table{%
x  y
-1.26290144016068 -0.929292917251587
-1.28471552365023 -0.848484873771667
-1.29358335367056 -0.767676770687103
-1.28999346870282 -0.686868667602539
-1.27374868801186 -0.60606062412262
-1.25252521038055 -0.547829409556484
-1.24344159824415 -0.525252521038055
-1.19573765850731 -0.444444447755814
-1.17171716690063 -0.41385314903138
-1.12419848760392 -0.363636374473572
-1.09090912342072 -0.334974077783273
-1.01133770098053 -0.282828271389008
-1.01010096073151 -0.282118175994636
-0.929292917251587 -0.248623509188058
-0.848484873771667 -0.229135420742136
-0.767676770687103 -0.222568333270994
-0.686868667602539 -0.228561386197583
-0.60606062412262 -0.247443902319774
-0.525252521038055 -0.280266676488917
-0.520734570028103 -0.282828271389008
-0.444444447755814 -0.332157501083179
-0.407527357257627 -0.363636374473572
-0.363636374473572 -0.409533711991383
-0.336007846056339 -0.444444447755814
-0.288124934108255 -0.525252521038055
-0.282828271389008 -0.538303236741772
-0.257969510062089 -0.60606062412262
-0.241698004636057 -0.686868667602539
-0.238102217201759 -0.767676770687103
-0.246984682187662 -0.848484873771667
-0.268834504625176 -0.929292917251587
-0.282828271389008 -0.961619514689719
-0.306223126107193 -1.01010096073151
-0.361720647866622 -1.09090912342072
-0.363636374473572 -1.09312123553085
-0.444444447755814 -1.16990722657157
-0.446924524293356 -1.17171716690063
-0.525252521038055 -1.22037053477544
-0.601615752891049 -1.25252521038055
-0.60606062412262 -1.25422926502263
-0.686868667602539 -1.27282559036751
-0.767676770687103 -1.27872786046488
-0.848484873771667 -1.27226024676559
-0.929292917251587 -1.25306749753533
-0.930682483612806 -1.25252521038055
-1.01010096073151 -1.21845577595455
-1.08440472603961 -1.17171716690063
-1.09090912342072 -1.16690619032566
-1.169937190561 -1.09090912342072
-1.17171716690063 -1.08872360123754
-1.22541103443375 -1.01010096073151
-1.25252521038055 -0.953421289478375
-1.26290144016068 -0.929292917251587
};
\addplot [draw=none, draw=red]
table{%
x  y
-1.01517795860897 -0.848484873771667
-1.03184207720296 -0.767676770687103
-1.02509612574488 -0.686868667602539
-1.01010096073151 -0.646702307488908
-0.989568191056005 -0.60606062412262
-0.929292917251587 -0.539768597638546
-0.907319841063044 -0.525252521038055
-0.848484873771667 -0.497575875924697
-0.767676770687103 -0.484668997482625
-0.686868667602539 -0.496447767217404
-0.623775557756085 -0.525252521038055
-0.60606062412262 -0.536601146533579
-0.541772039339364 -0.60606062412262
-0.525252521038055 -0.638155708093263
-0.506836233747155 -0.686868667602539
-0.500021681545232 -0.767676770687103
-0.516855196207306 -0.848484873771667
-0.525252521038055 -0.865281144682363
-0.569157614780741 -0.929292917251587
-0.60606062412262 -0.963084486552165
-0.686868667602539 -1.00671573852864
-0.706494057708888 -1.01010096073151
-0.767676770687103 -1.01820189007589
-0.823558171993629 -1.01010096073151
-0.848484873771667 -1.00538952123466
-0.929292917251587 -0.960358634860173
-0.962620951942466 -0.929292917251587
-1.01010096073151 -0.858768502657075
-1.01517795860897 -0.848484873771667
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={Posterior p(x₀|y)},
x grid style={darkgray176},
xlabel={X},
xmin=-4, xmax=4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Y},
ymin=-4, ymax=4,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-16.4387096774194, xmax=6.27096774193549, ymin=-5.32450331125828, ymax=5.27152317880795] {posterior_prior-005.png};
\end{groupplot}

\end{tikzpicture}


==> fig/dps_guidance_strength_fig/lpips_vs_cond_scaling_dps_15steps.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
height=\figureheight,
log basis x={10},
tick align=outside,
tick pos=left,
title={15 steps},
width=\figurewidth,
x grid style={darkgray176},
xlabel={Guidance strength},
xmajorgrids,
xmin=0.767270499010925, xmax=260.664264112613,
xminorgrids,
xmode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000},
xticklabels={
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\)
},
y grid style={darkgray176},
ylabel={LPIPS},
ymajorgrids,
ymin=0.531995388865471, ymax=0.644331303238869,
yminorgrids,
ytick style={color=black}
]
\addplot [thick, steelblue31119180, opacity=0.7, mark=none, mark size=3, mark options={solid}]
table {%
1 0.639225125312805
25 0.550586879253387
30 0.543354749679565
50 0.537101566791534
100 0.541972637176514
200 0.546619653701782
};
\end{axis}

\end{tikzpicture}


==> fig/dps_guidance_strength_fig/lpips_vs_cond_scaling_dps_30steps.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
height=\figureheight,
log basis x={10},
tick align=outside,
tick pos=left,
title={30 steps},
width=\figurewidth,
x grid style={darkgray176},
xlabel={Guidance strength},
xmajorgrids,
xmin=0.630957344480193, xmax=15848.9319246111,
xminorgrids,
xmode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000,100000,1000000},
xticklabels={
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\)
},
y grid style={darkgray176},
ylabel={LPIPS},
ymajorgrids,
ymin=0.437310057878494, ymax=0.646196168661118,
yminorgrids,
ytick style={color=black}
]
\addplot [thick, steelblue31119180, opacity=0.7, mark=none, mark size=3, mark options={solid}]
table {%
1 0.636701345443726
25 0.508968651294708
100 0.468388259410858
500 0.446804881095886
1000 0.449236303567886
2000 0.467687010765076
10000 0.532047510147095
};
\end{axis}

\end{tikzpicture}


==> fig/dps_guidance_strength_fig/lpips_vs_cond_scaling_dps_50steps.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
height=\figureheight,
log basis x={10},
tick align=outside,
tick pos=left,
title={50 steps},
width=\figurewidth,
x grid style={darkgray176},
xlabel={Guidance strength},
xmajorgrids,
xmin=0.630957344480193, xmax=15848.9319246111,
xminorgrids,
xmode=log,
xtick style={color=black},
xtick={0.01,0.1,1,10,100,1000,10000,100000,1000000},
xticklabels={
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\)
},
y grid style={darkgray176},
ylabel={LPIPS},
ymajorgrids,
ymin=0.395951396226883, ymax=0.642081373929977,
yminorgrids,
ytick style={color=black}
]
\addplot [thick, steelblue31119180, opacity=0.7, mark=none, mark size=3, mark options={solid}]
table {%
1 0.630893647670746
25 0.494640648365021
30 0.489161968231201
50 0.474424749612808
100 0.449130356311798
200 0.430458009243011
1000 0.407139122486115
3000 0.418687760829926
10000 0.451930165290833
};
\end{axis}

\end{tikzpicture}


==> fig/hyperparam_sweeps/dps_tuning.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

    \definecolor{darkgray176}{RGB}{176,176,176}
    
    \begin{groupplot}[group style={group size=2 by 4}]
    \nextgroupplot[
    height=\figureheight,
    tick align=outside,
    tick pos=left,
    title={15 steps, euler solver Best LPIPS scale: 100.00 Best SSIM scale: 50.00},
    width=\figurewidth,
    x grid style={darkgray176},
    xlabel={Conditioning Scale},
    xmajorgrids,
    xmin=-498.95, xmax=10499.95,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{blue}{LPIPS},
    ymajorgrids,
    ymin=0.555445405840874, ymax=0.650881257653236,
    ytick style={color=black}
    ]
    \addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
    table {%
    1 0.646543264389038
    25 0.584184110164642
    50 0.5763218998909
    100 0.559783399105072
    500 0.584455907344818
    1000 0.603956699371338
    2000 0.617452442646027
    10000 0.641854584217072
    };
    \draw (axis cs:0.02,0.98) node[
      scale=0.5,
      anchor=north west,
      text=blue,
      rotate=0.0
    ]{Best LPIPS: 100.00};
    \draw (axis cs:0.02,0.9) node[
      scale=0.5,
      anchor=north west,
      text=red,
      rotate=0.0
    ]{Best SSIM: 50.00};
    
    \nextgroupplot[
    height=\figureheight,
    tick align=outside,
    tick pos=left,
    title={15 steps, heun solver Best LPIPS scale: 80.00 Best SSIM scale: 80.00},
    width=\figurewidth,
    x grid style={darkgray176},
    xlabel={Conditioning Scale},
    xmajorgrids,
    xmin=-3.95, xmax=104.95,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{blue}{LPIPS},
    ymajorgrids,
    ymin=0.528934314846992, ymax=0.745894178748131,
    ytick style={color=black}
    ]
    \addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
    table {%
    1 0.736032366752625
    25 0.557071506977081
    50 0.546145260334015
    80 0.538796126842499
    100 0.5447136759758
    };
    \draw (axis cs:0.02,0.98) node[
      scale=0.5,
      anchor=north west,
      text=blue,
      rotate=0.0
    ]{Best LPIPS: 80.00};
    \draw (axis cs:0.02,0.9) node[
      scale=0.5,
      anchor=north west,
      text=red,
      rotate=0.0
    ]{Best SSIM: 80.00};
    
    \nextgroupplot[
    height=\figureheight,
    tick align=outside,
    tick pos=left,
    title={30 steps, euler solver Best LPIPS scale: 500.00 Best SSIM scale: 500.00},
    width=\figurewidth,
    x grid style={darkgray176},
    xlabel={Conditioning Scale},
    xmajorgrids,
    xmin=-498.95, xmax=10499.95,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{blue}{LPIPS},
    ymajorgrids,
    ymin=0.46035380512476, ymax=0.640159921348095,
    ytick style={color=black}
    ]
    \addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
    table {%
    1 0.631986916065216
    25 0.529033422470093
    50 0.510080218315125
    100 0.48447859287262
    500 0.468526810407639
    1000 0.484384924173355
    2000 0.505902588367462
    10000 0.561822235584259
    };
    \draw (axis cs:0.02,0.98) node[
      scale=0.5,
      anchor=north west,
      text=blue,
      rotate=0.0
    ]{Best LPIPS: 500.00};
    \draw (axis cs:0.02,0.9) node[
      scale=0.5,
      anchor=north west,
      text=red,
      rotate=0.0
    ]{Best SSIM: 500.00};
    
    \nextgroupplot[
    height=\figureheight,
    tick align=outside,
    tick pos=left,
    title={30 steps, heun solver Best LPIPS scale: 500.00 Best SSIM scale: 500.00},
    width=\figurewidth,
    x grid style={darkgray176},
    xlabel={Conditioning Scale},
    xmajorgrids,
    xmin=-498.95, xmax=10499.95,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{blue}{LPIPS},
    ymajorgrids,
    ymin=0.431896357238293, ymax=0.646700800955296,
    ytick style={color=black}
    ]
    \addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
    table {%
    1 0.636936962604523
    25 0.510440826416016
    50 0.488652497529984
    100 0.465513408184052
    500 0.441660195589065
    1000 0.445562064647675
    2000 0.469718933105469
    10000 0.530877292156219
    };
    \draw (axis cs:0.02,0.98) node[
      scale=0.5,
      anchor=north west,
      text=blue,
      rotate=0.0
    ]{Best LPIPS: 500.00};
    \draw (axis cs:0.02,0.9) node[
      scale=0.5,
      anchor=north west,
      text=red,
      rotate=0.0
    ]{Best SSIM: 500.00};
    
    \nextgroupplot[
    height=\figureheight,
    tick align=outside,
    tick pos=left,
    title={50 steps, euler solver Best LPIPS scale: 1000.00 Best SSIM scale: 500.00},
    width=\figurewidth,
    x grid style={darkgray176},
    xlabel={Conditioning Scale},
    xmajorgrids,
    xmin=-447.5, xmax=10497.5,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{blue}{LPIPS},
    ymajorgrids,
    ymin=0.413350009918213, ymax=0.487346267700195,
    ytick style={color=black}
    ]
    \addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
    table {%
    50 0.483982801437378
    100 0.465865075588226
    500 0.421650469303131
    1000 0.41671347618103
    2000 0.425319850444794
    10000 0.47999095916748
    };
    \draw (axis cs:0.02,0.98) node[
      scale=0.5,
      anchor=north west,
      text=blue,
      rotate=0.0
    ]{Best LPIPS: 1000.00};
    \draw (axis cs:0.02,0.9) node[
      scale=0.5,
      anchor=north west,
      text=red,
      rotate=0.0
    ]{Best SSIM: 500.00};
    
    \nextgroupplot[
    height=\figureheight,
    tick align=outside,
    tick pos=left,
    title={50 steps, heun solver Best LPIPS scale: 2000.00 Best SSIM scale: 1000.00},
    width=\figurewidth,
    x grid style={darkgray176},
    xlabel={Conditioning Scale},
    xmajorgrids,
    xmin=-447.5, xmax=10497.5,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{blue}{LPIPS},
    ymajorgrids,
    ymin=0.40333955436945, ymax=0.475570897758007,
    ytick style={color=black}
    ]
    \addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
    table {%
    50 0.472287654876709
    100 0.447350710630417
    500 0.415969043970108
    1000 0.408638030290604
    2000 0.406622797250748
    10000 0.453312784433365
    };
    \draw (axis cs:0.02,0.98) node[
      scale=0.5,
      anchor=north west,
      text=blue,
      rotate=0.0
    ]{Best LPIPS: 2000.00};
    \draw (axis cs:0.02,0.9) node[
      scale=0.5,
      anchor=north west,
      text=red,
      rotate=0.0
    ]{Best SSIM: 1000.00};
    
    \nextgroupplot[
    height=\figureheight,
    tick align=outside,
    tick pos=left,
    title={100 steps, euler solver Best LPIPS scale: 2000.00 Best SSIM scale: 2000.00},
    width=\figurewidth,
    x grid style={darkgray176},
    xlabel={Conditioning Scale},
    xmajorgrids,
    xmin=-447.5, xmax=10497.5,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{blue}{LPIPS},
    ymajorgrids,
    ymin=0.384584295749664, ymax=0.469674956798553,
    ytick style={color=black}
    ]
    \addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
    table {%
    50 0.465807199478149
    100 0.447225093841553
    500 0.40666002035141
    1000 0.396541744470596
    2000 0.388452053070068
    10000 0.412442147731781
    };
    \draw (axis cs:0.02,0.98) node[
      scale=0.5,
      anchor=north west,
      text=blue,
      rotate=0.0
    ]{Best LPIPS: 2000.00};
    \draw (axis cs:0.02,0.9) node[
      scale=0.5,
      anchor=north west,
      text=red,
      rotate=0.0
    ]{Best SSIM: 2000.00};
    
    \nextgroupplot[
    height=\figureheight,
    tick align=outside,
    tick pos=left,
    title={100 steps, heun solver Best LPIPS scale: 2000.00 Best SSIM scale: 2000.00},
    width=\figurewidth,
    x grid style={darkgray176},
    xlabel={Conditioning Scale},
    xmajorgrids,
    xmin=-447.5, xmax=10497.5,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{blue}{LPIPS},
    ymajorgrids,
    ymin=0.384932424128056, ymax=0.46350050419569,
    ytick style={color=black}
    ]
    \addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
    table {%
    50 0.459929227828979
    100 0.438816249370575
    500 0.401726186275482
    1000 0.391157180070877
    2000 0.388503700494766
    10000 0.410945564508438
    };
    \draw (axis cs:0.02,0.98) node[
      scale=0.5,
      anchor=north west,
      text=blue,
      rotate=0.0
    ]{Best LPIPS: 2000.00};
    \draw (axis cs:0.02,0.9) node[
      scale=0.5,
      anchor=north west,
      text=red,
      rotate=0.0
    ]{Best SSIM: 2000.00};
    \end{groupplot}
    
    \begin{groupplot}[group style={group size=2 by 4}]
    \nextgroupplot[
    axis y line=right,
    height=\figureheight,
    tick align=outside,
    width=\figurewidth,
    x grid style={darkgray176},
    xmin=-498.95, xmax=10499.95,
    xtick pos=left,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{red}{SSIM},
    ymin=0.305931195616722, ymax=0.466077581048012,
    ytick pos=right,
    ytick style={color=black},
    yticklabel style={anchor=west}
    ]
    \addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
    table {%
    1 0.363336682319641
    25 0.447610348463058
    50 0.458798199892044
    100 0.455206274986267
    500 0.414973497390747
    1000 0.388695240020752
    2000 0.361166000366211
    10000 0.31321057677269
    };
    
    \nextgroupplot[
    axis y line=right,
    height=\figureheight,
    tick align=outside,
    width=\figurewidth,
    x grid style={darkgray176},
    xmin=-3.95, xmax=104.95,
    xtick pos=left,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{red}{SSIM},
    ymin=0.212724063545465, ymax=0.458935718983412,
    ytick pos=right,
    ytick style={color=black},
    yticklabel style={anchor=west}
    ]
    \addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
    table {%
    1 0.223915502429008
    25 0.428087502717972
    50 0.445254594087601
    80 0.447744280099869
    100 0.447174817323685
    };
    
    \nextgroupplot[
    axis y line=right,
    height=\figureheight,
    tick align=outside,
    width=\figurewidth,
    x grid style={darkgray176},
    xmin=-498.95, xmax=10499.95,
    xtick pos=left,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{red}{SSIM},
    ymin=0.340029217302799, ymax=0.540128521621227,
    ytick pos=right,
    ytick style={color=black},
    yticklabel style={anchor=west}
    ]
    \addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
    table {%
    1 0.349124640226364
    25 0.484249472618103
    50 0.504349827766418
    100 0.520646214485168
    500 0.531033098697662
    1000 0.506103694438934
    2000 0.485132336616516
    10000 0.42034062743187
    };
    
    \nextgroupplot[
    axis y line=right,
    height=\figureheight,
    tick align=outside,
    width=\figurewidth,
    x grid style={darkgray176},
    xmin=-498.95, xmax=10499.95,
    xtick pos=left,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{red}{SSIM},
    ymin=0.309648376703262, ymax=0.546017545461655,
    ytick pos=right,
    ytick style={color=black},
    yticklabel style={anchor=west}
    ]
    \addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
    table {%
    1 0.320392429828644
    25 0.470111548900604
    50 0.494433492422104
    100 0.516018927097321
    500 0.535273492336273
    1000 0.530101716518402
    2000 0.508328676223755
    10000 0.464828908443451
    };
    
    \nextgroupplot[
    axis y line=right,
    height=\figureheight,
    tick align=outside,
    width=\figurewidth,
    x grid style={darkgray176},
    xmin=-447.5, xmax=10497.5,
    xtick pos=left,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{red}{SSIM},
    ymin=0.497974136471748, ymax=0.581912359595299,
    ytick pos=right,
    ytick style={color=black},
    yticklabel style={anchor=west}
    ]
    \addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
    table {%
    50 0.516465544700623
    100 0.540138602256775
    500 0.578096985816956
    1000 0.577833116054535
    2000 0.569916725158691
    10000 0.501789510250092
    };
    
    \nextgroupplot[
    axis y line=right,
    height=\figureheight,
    tick align=outside,
    width=\figurewidth,
    x grid style={darkgray176},
    xmin=-447.5, xmax=10497.5,
    xtick pos=left,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{red}{SSIM},
    ymin=0.504847526550293, ymax=0.580449342727661,
    ytick pos=right,
    ytick style={color=black},
    yticklabel style={anchor=west}
    ]
    \addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
    table {%
    50 0.508283972740173
    100 0.530440807342529
    500 0.565861821174622
    1000 0.577012896537781
    2000 0.575941264629364
    10000 0.546611607074738
    };
    
    \nextgroupplot[
    axis y line=right,
    height=\figureheight,
    tick align=outside,
    width=\figurewidth,
    x grid style={darkgray176},
    xmin=-447.5, xmax=10497.5,
    xtick pos=left,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{red}{SSIM},
    ymin=0.515439948439598, ymax=0.617766955494881,
    ytick pos=right,
    ytick style={color=black},
    yticklabel style={anchor=west}
    ]
    \addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
    table {%
    50 0.52009117603302
    100 0.545770287513733
    500 0.592258095741272
    1000 0.604031324386597
    2000 0.613115727901459
    10000 0.596087694168091
    };
    
    \nextgroupplot[
    axis y line=right,
    height=\figureheight,
    tick align=outside,
    width=\figurewidth,
    x grid style={darkgray176},
    xmin=-447.5, xmax=10497.5,
    xtick pos=left,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel=\textcolor{red}{SSIM},
    ymin=0.510240626335144, ymax=0.610076355934143,
    ytick pos=right,
    ytick style={color=black},
    yticklabel style={anchor=west}
    ]
    \addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
    table {%
    50 0.514778614044189
    100 0.539410710334778
    500 0.583388209342957
    1000 0.592871904373169
    2000 0.605538368225098
    10000 0.59794157743454
    };
    \end{groupplot}
    
    
    \end{tikzpicture}
    
